On Riemannian Stochastic Approximation Schemes with Fixed Step-Size

This paper studies fixed step-size stochastic approximation (SA) schemes, including stochastic gradient schemes, in a Riemannian framework. It is motivated by several applications, where geodesics can be computed explicitly, and their use accelerates crude Euclidean methods. A fixed step-size scheme defines a family of time-homogeneous Markov chains, parametrized by the step-size. Here, using this formulation, non-asymptotic performance bounds are derived, under Lyapunov conditions. Then, for any step-size, the corresponding Markov chain is proved to admit a unique stationary distribution, and to be geometrically ergodic. This result gives rise to a family of stationary distributions indexed by the step-size, which is further shown to converge to a Dirac measure, concentrated at the solution of the problem at hand, as the step-size goes to 0. Finally, the asymptotic rate of this convergence is established, through an asymptotic expansion of the bias, and a central limit theorem.

==> notations.tex <==
\paragraph{Notations}
For any $\theta \in \Theta$ and $v,w \in \planT_\theta \Theta$, denote
by $\frg_\theta(v,w)=\psr{v}{w}[\theta]$ and its corresponding norm by
$\frg_\theta(v,v)=\normr{v}[\theta]^2$.
$\distT:\Theta \times \Theta \to \rset_+$ denotes the distance
associated with the Riemannian metric $\frg$.  For any
$\theta_0 \in \Theta,r>0$, set
$\ball{\theta_0}{r}=\defEnsLigne{\theta_1 \in \Theta \,:\,
  \distT(\theta_0,\theta_1)<r}$, the open ball centered at $\theta_0$
with radius $r$. Similarly, we define closed balls in $\Theta$ by
$\cball{\theta_0}{r}=\defEnsLigne{\theta_1 \in \Theta \,:\,
  \distT(\theta_0,\theta_1)\leq r}$.

For a smooth function $g:\Theta \to \rset$, we denote by $\grad g$ its Riemannian gradient \cite[p. 27]{lee:2019} and by $\Hess g$ its Riemannian, or covariant, Hessian \cite[Example 4.22]{lee:2019}. 
For a curve $\upgamma:I \to \Theta, \parallelTransport_{t_0,t_1}^\upgamma : \planT_{\upgamma(t_0)} \Theta \to \planT_{\upgamma(t_1)} \Theta$ stands for the parallel transport map associated to the Levi-Civita connection along $\upgamma$ from $\upgamma(t_0)$ to $\upgamma(t_1)$ \cite[Equation 4.22]{lee:2019}. 
Moreover, for any $\theta\in \Theta$, under the assumption that $\Theta$ is complete, 
consider the Riemannian exponential map $\Exp_{\theta} : \planT_\theta \Theta \to \Theta$,
see \cite[Proposition 5.19]{lee:2019}.
This map projects a vector from
the tangent space $T_\theta\Theta$ onto the manifold $\Theta$, following a geodesic curve.

% In this context, let $\proj_\mss : \Theta \to \mss$ be the projection on $\mss$, see \cite[Proposition 2.6]{sturm:2003}.
%For any $\theta \in \Theta$, if $A,B:\planT_\theta \Theta \times \planT_\theta \Theta \to \rset$ are bilinear and symmetric forms, we say $A \preceq B$ when $B-A$ is positive semi-definite, and say $A \prec B$ when $B-A$ is positive definite. These definitions are extended to self-adjoint operators $E:\planT_\theta \Theta \to \planT_\theta \Theta$ by considering the bilinear and symmetric form on $\planT_\theta \Theta \times \planT_\theta \Theta$ defined by $v,w \mapsto \psr{Ev}{w}[\theta]$.
Finally, denote $\Leb_\theta$ the Lebesgue measure on $\planT_\theta \Theta$ for any $\theta \in \Theta$.
% and $\wedge$ for the minimum of two real numbers.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> table_assumptions.tex <==

%\vspace{-1.8cm}
\section{Assumptions}
\subsection*{On the manifold}
\begin{assumptionA}
Assume one of the following conditions.
\begin{enumerate}[wide, labelwidth=!, labelindent=0pt,label=(\roman*),noitemsep,nolistsep]
\item $\Theta$ is a Hadamard manifold, \ie~a complete, simply connected Riemannian manifold with non-positive sectional curvature. In addition, $\mss$ is a closed geodesically convex subset of $\Theta$ with non-empty interior.
\item $\Theta$ is a complete, connected Riemannian manifold and $\mss=\Theta$.
\end{enumerate}
\end{assumptionA}

\begin{assumptionA} 
 $\Theta$ is a Hadamard manifold. In addition, there exists $\kappa > 0$ such that the sectional curvature of $\Theta$ is bounded below by $- \kappa^2$.
\end{assumptionA}
\subsection*{On the distribution of the data}
\begin{assumptionMD}
  The sequence $(X_n)_{n \in \nsets}$ is  independent and identically distributed (\iid). In addition, for any $\theta \in\Theta$, $\expe{\noise_{\theta}(X_{1})} = 0$ and there exist $\sigmaZ,\sigmaU > 0$ such that 
for any $\theta \in \mss$, $\expeLigne{\normrLigne{\noise_{\theta}\parenthese{X_{1}}}[\theta]^2 } \leq \sigmaZ + 
\sigmaU\, \normr{h(\theta)}[\theta]^2$.
% \begin{equation}
% \expe{\normr{\noise_{\theta}\parenthese{X_{1}}}[\theta]^2 } \leq \sigmaZ + 
% \sigmaU\, \normr{h(\theta)}[\theta]^2 \eqsp.
% \end{equation}
\end{assumptionMD}
\begin{assumptionMD}
  \begin{enumerate}[wide, labelwidth=!, labelindent=0pt,label=(\roman*),noitemsep,nolistsep]
\item 
$\PP$-almost surely,  the vector field $\theta \mapsto \noise_{\theta}(X_1)$ is  continuous on $\Theta$. 
\item  
 For any $\theta \in \Theta$, $\Leb_\theta$ and the distribution of $\noise_\theta(X_1)$ are mutually absolutely continuous. 
  \end{enumerate}
\end{assumptionMD}

\begin{assumptionMD} $\Sigma$ is a continuous
  tensor field of type $(2,0)$ on $\Theta$.
\end{assumptionMD}
\begin{assumptionMD}
   There exist
  $\varepsilon_e >0$, $\tsigma_{0}^2,\tsigma_{1}^2 \geq 0$ such that for any $\theta \in \Theta$, $\PE[\normr{e_{\theta}(X_1)}[\theta]^{2+\varepsilon_e}] \leq \tsigma_0^2 + \tsigma_1^2 V(\theta)$.
\end{assumptionMD}

\begin{assumptionMD}
%  \label{ass:second_moment_pi}
  There exists $\theta \in \Theta$ such that
  \begin{equation}
    \label{eq:2}
    \int_{\Theta} \distT^2(\theta,\nu) \pi (\rmd \nu) < \plusinfty \eqsp.
  \end{equation}
\end{assumptionMD}

\subsection*{On the Lyapunov function $V$ and the mean field function $h$}
\begin{assumption}
\begin{enumerate}[wide, labelwidth=!, labelindent=0pt,label=(\roman*),noitemsep,nolistsep]
\item For any $\theta\in \Theta$, $V\circ\proj_\mss(\theta) \leq V(\theta)$.
\item $V$ is continuously differentiable on $\Theta$ and its Riemannian gradient $\grad V$ is geodesically $L$-Lipschitz, \ie, there exists $L \geq 0$ such that for any $\theta_0,\theta_1 \in \Theta$, and geodesic curve $\upgamma:[0,1]\to \Theta$ such that $\upgamma(0)=\theta_0$ and $\upgamma(1)=\theta_1$, 
\begin{equation}
\normr{\grad V(\theta_1)- \parallelTransport_{01}^{\upgamma} \grad V(\theta_0)}[\theta_1] \leq L \ell(\upgamma) \eqsp ,
\end{equation}  
where $\ell(\upgamma)=\normrLigne{\dot{\upgamma}(0)}[\theta_0]$ is the length of the geodesic.
\item $V$ is proper on $\mss$,
  \ie, for any $M \geq 0$, there exists a compact set
  $\msk \subset \mss$ such that for any $\theta \in \mss \setminus \msk$, $V(\theta) > M$. 
\end{enumerate}
\end{assumption}
\begin{assumption}
  There exist $C_1 \geq 0$ and $C_2>0$ such that for any $\theta \in \mss$, $\normr{h(\theta)}[\theta]^2 + C_2 \psr{\grad V(\theta)}{h(\theta)}[\theta] \leq C_1$.
\end{assumption}

\begin{assumption}[$\msks$] 
  There exists $\lambda>0$  such that for any $\theta \in \mss$, $\psr{\grad V(\theta)}{h(\theta)}[\theta] \leq - \lambda V(\theta)\1_{\mss \setminus \msks}(\theta)$.
\end{assumption}

\begin{assumption}
There exists
  $\thetas \in \mss$ such that for any $r >0$,
  \Cref{ass:lyap_minorization}$(\cball{\thetas}{r})$ holds and that
  there exists $c_r>0$ satisfying for any
  $\theta \in \mss \setminus \cball{\thetas}{r}$, $c_r \leq V(\theta)$.
\end{assumption}
\begin{assumption} 
 There exist a linear mapping $\bfA: \planT_{\theta^*}\Theta \rightarrow \planT_{\theta^*}\Theta$ and a map $\scrH:\Theta \to \planT_{\theta^*} \Theta$, such that for any $\theta \in \Theta$,
\begin{equation} 
 h(\theta) = \parallelTransport_{01}^{\upgamma}\left( \bfA \Exp^{-1}_{\thetas}(\theta) + \scrH(\theta)\right)\eqsp,
\end{equation}
where $\thetas$ is defined in \Cref{ass:V_positive}, $\parallelTransport_{01}^{\upgamma}$ denotes parallel transport along the geodesic $\upgamma :[0,1]\rightarrow \Theta$ with $\upgamma(0) = \thetas$ and $\upgamma(1) = \theta$, and $\lim_{\theta \to \thetas} \defEnsLigne{\normr{\scrH(\theta)}[\thetas]/\distT(\thetas,\theta)}=0$.
In addition, % 
 the eigenvalues of the matrix $\bfA$ all have strictly negative real parts. Finally, there exists $C_3 > 0$ such that for any
  $\theta \in \Theta$,
  $\normr{h(\theta)}[\theta] \leq C_3 \distT(\thetas,\theta)$.
\end{assumption}

\begin{assumption}
  There exists $\thetas$ such that
  \Cref{ass:lyap_minorization}$(\{\thetas\})$ holds and there exists
  $\phi : \rset_+ \to \rset_+$ such that for any $\theta \in \Theta$,
  $V(\theta) \geq \phi(\distT(\thetas,\theta))$ and for any $r >0$,
  $\inf_{\coint{r,\plusinfty}}\phi >0$. In addition, there exists $\bar{a} >0$,
  such that $\lim_{r\to \plusinfty} \sup_{a \leq \bar{a}} a/\phi(a^{1/2}r) =
  0$. 
\end{assumption}
\subsection*{On the objective function $f$ in the gradient case}
\begin{assumptionF}
  $f : \Theta \to \rset$ is twice continuously differentiable and $\grad f$ is geodesically $L_f$-Lipschitz, see \eqref{eq:llipschitz}. 
\end{assumptionF}

\begin{assumptionF} 
   $f$ is $\lambda_f$-strongly geodesically convex, for
  some $\lambda_f > 0$, \ie~for any $\theta_1,\theta_2 \in \Theta$,
  $f(\theta_2) \geq f(\theta_1) +
  \psrLigne{\Exp_{\theta_1}^{-1}(\theta_2)}{\grad f(\theta_1)}[\theta_1] +
  \lambda_f\distT^2(\theta_1,\theta_2)/2$.
\end{assumptionF}
\begin{assumptionF} $f$ is twice continuously differentiable. There exists $\tlambda_f >0$
  such that for any $\theta \in \Theta$,
  $ -\psrLigne{\Exp^{-1}_\theta(\thetas)}{\grad f(\theta)}[\theta] \geq \tlambda_f
  V_1(\theta) $, where $V_1$ is defined by \eqref{eq:lyapunovV} with
  $\delta =1$. In addition, there exists $C_f > 0$ such that for any
  $\theta \in \Theta$,
  $\normr{\grad f(\theta)}[\theta]^2 \leq C_f
  (\distT^2(\thetas,\theta) \wedge 1)$.
\end{assumptionF}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_supplement"
%%% End:

